Predictive Data Race Detection for GPUs

The high degree of parallelism and relatively complicated synchronization mechanisms in GPUs make writing correct kernels difficult. Data races pose one such concurrency correctness challenge, and therefore, effective methods of detecting as many data races as possible are required. Predictive partial order relations for CPU programs aim to expose data races that can be hidden during a dynamic execution. Existing predictive partial orders cannot be na\"ively applied to analyze GPU kernels because of the differences in programming models. This work proposes GWCP, a predictive partial order for data race detection of GPU kernels. GWCP extends a sound and precise relation called weak-causally-precedes (WCP) proposed in the context of multithreaded shared memory CPU programs to GPU kernels. GWCP takes into account the GPU thread hierarchy and different synchronization semantics such as barrier synchronization and scoped atomics and locks. We implement a tool called PreDataR that tracks the GWCP relation using binary instrumentation. PreDataR includes three optimizations and a novel vector clock compression scheme that are readily applicable to other partial order based analyses. Our evaluation with several microbenchmarks and benchmarks shows that PreDataR has better data race coverage compared to prior techniques at practical run-time overheads.

==> algo-wcp-acm.tex <==
\begin{small}
    \begin{algorithm}[t]
        \label{algo:gwcp-acm}
        \caption{Tracking \GWCP for race detection on GPUs}
        \begin{algorithmic}[1]
            % Barrier

            \Procedure{sync}{scope}
            \State $joined \leftarrow VC()$
            \State $joined_{HB} \leftarrow VC()$

            \ForAll {$t \in$ scope}
            \State $\mathbb{C}_t \coloneqq \mathbb{P}_t\{t\coloneqq \mathbb{N}_t\}$
            \State $joined \coloneqq joined \sqcup \mathbb{C}_t$
            \State $joined_{HB} \coloneqq joined_{HB} \sqcup \mathbb{H}_t$
            \EndFor

            \ForAll {$t \in$ scope}
            \State $\mathbb{P}_t \coloneqq joined$
            \State $\mathbb{H}_t \coloneqq joined_{HB}$
            \EndFor

            \State $\mathbb{N}_t \coloneqq \mathbb{N}_t + 1$
            \State $increment(\mathbb{H}_t)$
            \EndProcedure


            % Acquire

            \Procedure{acquire}{$t$, $l$, $s$}
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{P}_{<l,s>}$
            \State $\mathbb{H}_t \coloneqq \mathbb{H}_t \sqcup \mathbb{H}_{<l,s>}$
            \If {$s$ = 0}
            \ForAll {$block \in grid$}
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{P}_{<l,block+1>}$
            \State $\mathbb{H}_t \coloneqq \mathbb{H}_t \sqcup \mathbb{H}_{<l,block+1>}$
            \EndFor
            \Else
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{P}_{<l,0>}$
            \State $\mathbb{H}_t \coloneqq \mathbb{H}_t \sqcup \mathbb{H}_{<l,0>}$
            \EndIf
            \ForAll {$t' \neq t$}
            \State Acq$_l(t')$.enque$(<\mathbb{C}_t, s>)$
            \EndFor
            \EndProcedure

            % Release

            \Procedure{release}{$t$, $l$, $R$, $W$, $s$}
            \While{Acq$_l(t)$.front$()$ $\sqsubseteq \mathbb{C}_t$}
            \State Acq$_l(t)$.deque()
            \State <VC, scope> $\leftarrow$ Rel$_l(t)$.deque()

            \If {$scope$ = 0 \Or  $scope$ = $block(t)$ + 1}
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup$ $VC$
            \EndIf
            \EndWhile
            \ForAll {$x \in R$}
            \State $\mathbb{L}_{<l,s>, x}^r \coloneqq \mathbb{L}_{<l,s>, x}^r \sqcup \mathbb{H}_t$
            \EndFor
            \ForAll {$x \in W$}
            \State $\mathbb{L}_{<l,s>, x}^w \coloneqq \mathbb{L}_{<l,s>, x}^w \sqcup \mathbb{H}_t$
            \EndFor
            \State $\mathbb{H}_{<l,s>} \coloneqq \mathbb{H}_t$
            \State $\mathbb{P}_{<l,s>} \coloneqq \mathbb{P}_t$
            \ForAll {$t' \neq t$}
            \State Rel$_l(t')$.enque$(<\mathbb{H}_t,s>)$
            \EndFor
            \State $\mathbb{N}_t \coloneqq \mathbb{N}_t + 1$
            \State $increment(\mathbb{H}_t)$
            \EndProcedure

            % Read

            \Procedure{read}{$t$, $x$, $L$}
            \ForAll {$<l, s> \in L$}
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{L}_{<l,s>, x}^w$
            \If {$s$ = 0}
            \ForAll {$block \in grid$}
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{L}_{<l, block+1>, x}^w$
            \EndFor
            \Else
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{L}_{<l, 0>, x}^w$
            \EndIf
            \EndFor
            \EndProcedure

            % Write

            \Procedure{write}{$t$, $x$, $L$}
            \ForAll {$<l, s> \in L$}
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{L}_{<l,s>, x}^w$
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{L}_{<l,s>, x}^r$
            \If {$s$ = 0}
            \ForAll {$block \in grid$}
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{L}_{<l, block+1>, x}^w$
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{L}_{<l, block+1>, x}^r$
            \EndFor
            \Else
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{L}_{<l, 0>, x}^w$
            \State $\mathbb{P}_t \coloneqq \mathbb{P}_t \sqcup \mathbb{L}_{<l, 0>, x}^r$
            \EndIf
            \EndFor
            \EndProcedure

        \end{algorithmic}
    \end{algorithm}
\end{small}

\swarnendu{Algorithm~\ref{algo:gwcp-acm} Fix line 10, scope=0 has no meaning. Line 21: What is s? Add a few comments to explain the steps.}


==> chktexrc <==
# see /usr/local/texlive/*/texmf-dist/chktex/chktexrc for all defaults

# call like `chktex -v2 -g -l ~/.chktexrc paper.tex` to get local config to overwrite global

# if you get the message, "WARNING -- ChkTeX does not handle lines over 1021 bytes correctly",
# you might find this regular expression handy: [^\n]{1021,}

# supposedly this is the default and it's in the global chktexrc but doesn't work unless repeated here
# QuoteStyle = Traditional #=> "An example," he said, "would be great."
# QuoteStyle = Logical     #=> "An example", he said, "would be great".
QuoteStyle = Logical

TabSize = 2

# -v2 means fancy error display
# but for some reason we can't use it here; it has to go before the other command line options, i.e., -g
# CmdLine
# {
#     -v
# }

# Allow only "-" and "---" separators inside words
HyphDash
{
    1 3
}

# Allow only "--" separators between numbers (the global default)
NumDash
{
    2
}

# Disallow all usage of " --- ", " -- ", or " - "
WordDash
{
    0
}

# ignore "Command terminated with space" warnings for these commands:
Silent
{
    \begingroup
    \centering
    \dash
    \dots
    \draw
    \endgroup
    \endinput
    \footnotemark
    \hfil
    \hfill
    \item
    \ldots
    \linebreak
    \makeappendix
    \makeatletter
    \makeatother
    \maketableofcontents
    \maketitle
    \medskip
    \newline
    \node
    \noindent
    \path
    \phantomsection
    \printbibliography
    \quad
    \today
# math operators
    \approx
    \geq
    \neg
    \supset
    \wedge
# size commands
    \tiny
    \scriptsize
    \footnotesize
    \small
    \normalsize
    \large
    \Large
    \LARGE
    \huge
    \Huge
# booktabs
    \bottomrule
    \midrule
    \toprule
# caption/subcaption/subfig packages
    \ContinuedFloat
}


==> fig-lockset-false-positive.tex <==
\begin{figure}[t]
    \centering
    % \begin{small}
    \begin{minipage}[t]{0.15\linewidth}
        \textbf{Event}
        \begin{lstlisting}[style=TraceStyle]
e1
e2
e3
        \end{lstlisting}
    \end{minipage}%
    \begin{minipage}[t]{0.35\linewidth}
        \textbf{Thread 1}
        \begin{lstlisting}[style=TraceStyle]
wr(x)
barrier


        \end{lstlisting}
    \end{minipage}%
    \begin{minipage}[t]{0.35\linewidth}
        \textbf{Thread 2}
        \begin{lstlisting}[style=TraceStyle]

barrier
wr(x)
        \end{lstlisting}
    \end{minipage}
    % \end{small}
    \caption{An example of a false race report with lockset detection.}
    \label{fig:lockset-false-positive}
\end{figure}


==> fig-predictable-race-smarttrack.tex <==
\begin{figure}
    \centering
    % \begin{small}
    \begin{minipage}[t]{0.15\linewidth}
        \textbf{Event}
        \begin{lstlisting}[style=TraceStyle]
e1
e2
e3
e4
e5
e6
e7
e8
e9
e10
e11
e12
            \end{lstlisting}
    \end{minipage}%
    % \hfill
    \begin{minipage}[t]{0.28\linewidth}
        \textbf{Thread 1}
        \begin{lstlisting}[style=TraceStyle]
wr(x)
acq(m)
wr(y)
rel(m)








        \end{lstlisting}
    \end{minipage}%
    % \hfill
    \begin{minipage}[t]{0.28\linewidth}
        \textbf{Thread 2}
        \begin{lstlisting}[style=TraceStyle]




acq(m)
wr(y)
rel(m)
acq(n)
rel(n)






        \end{lstlisting}
    \end{minipage}%
    % \hfill
    \begin{minipage}[t]{0.28\linewidth}
        \textbf{Thread 3}
        \begin{lstlisting}[style=TraceStyle]









acq(n)
rel(n)
wr(x)
        \end{lstlisting}
    \end{minipage}
    % \end{small}
    \caption{Predictable race missed by both ScoRD and Barracuda algorithms}
    \label{fig:predictable-race-smarttrack}
\end{figure}


==> fig-predictable-wcp.tex <==
\begin{figure}[t]
    \centering
    % \begin{small}
    \begin{minipage}[t]{0.15\linewidth}
        \textbf{Event}
        \begin{lstlisting}[style=TraceStyle]
e1
e2
e3
e4
e5
e6
e7
e8
e9
e10
e11
e12
            \end{lstlisting}
    \end{minipage}%
    % \hfill
    \begin{minipage}[t]{0.28\linewidth}
        \textbf{Thread 1}
        \begin{lstlisting}[style=TraceStyle]
acq(l)
sync(x)
rd(z)
rel(l)








        \end{lstlisting}
    \end{minipage}%
    % \hfill
    \begin{minipage}[t]{0.28\linewidth}
        \textbf{Thread 2}
        \begin{lstlisting}[style=TraceStyle]




sync(x)
acq(l)
acq(n)
rel(n)
rel(l)






        \end{lstlisting}
    \end{minipage}%
    % \hfill
    \begin{minipage}[t]{0.28\linewidth}
        \textbf{Thread 3}
        \begin{lstlisting}[style=TraceStyle]









acq(n)
rel(n)
wr(z)
        \end{lstlisting}
    \end{minipage}
    % \end{small}
    \caption{HB tracking cannot detect the predictable race on \pcode{z} (events \pcode{e3} and \pcode{e12}). The predictable race is caught by WCP and \gwcp (\Cref*{sec:design-overview}).}
    \label{fig:predictable-race-wcp}
\end{figure}


==> fig-volatile-release.tex <==
\begin{figure}
    \centering
    % \begin{small}
    \begin{minipage}[t]{0.15\linewidth}
        \textbf{Event}
        \begin{lstlisting}[style=TraceStyle]
e1
e2
e3
e4
e5
e6
e7
        \end{lstlisting}
    \end{minipage}%
    \begin{minipage}[t]{0.35\linewidth}
        \textbf{Thread 1}
        \begin{lstlisting}[style=TraceStyle]
acq(m)
wr(x)
altrel(m)



wr(x)
        \end{lstlisting}
    \end{minipage}%
    \begin{minipage}[t]{0.35\linewidth}
        \textbf{Thread 2}
        \begin{lstlisting}[style=TraceStyle]



acq(m)
wr(x)
rel(m)
        \end{lstlisting}
    \end{minipage}
    % \end{small}
    % \swarnendu{Should we use CUDA syntax for this example? That might eat up more vertical space though.}
    \caption{Lockset analysis will not report the race between events \pcode{e5} and \pcode{e7} on \code{x} if %the pattern
        \small{\pcode{altrel(m)}} is not inferred as a lock release.}
    \label{fig:volatile-release}
\end{figure}


==> microbenchmarks.tex <==
\subsection{Predictive Microbenchmarks}
\label{sec:predictive-microbenchmarks}

The \barracuda and \scor benchmarks do not emphasize including predictable races. So, we have created a set of microbenchmarks that demonstrate the shortcomings of \barracuda and \scord. Our microbenchmark suite consists of XYZ kernel programs.

\swarnendu{Include a couple of new or concrete CUDA examples from the predictable test cases.}

\swarnendu{Should we move this to \Cref{sec:eval:setup}?}


==> tab-benchmarks.tex <==
\begin{small}
    \begin{table}
        \centering
        \begin{tabular}{lrr}
                             & \textbf{Grid size} & \textbf{Input}                                                \\
            \toprule
            \bench{\conv}    & <15,1024>          & data/scord/1dconv                                             \\
            \bench{\mm}      &                    &                                                               \\
            \bench{\red}     & <30,512>           & data/scord/reduction                                          \\
            \bench{\ruleone} & <15,1024>          & data/scord/rule-110                                           \\
            \bench{\uts}     &                    &                                                               \\

            \midrule

            \bench{\hotspot} &                    & 512 2 2 data/temp$\_$512 data/power$\_$512 hotspot$\_$out.out \\
            \bench{\kmeans}  &                    & -i data/kdd$\_$cup                                            \\
            \bench{\needle}  &                    & 2048 10                                                       \\
            \bench{\pf}      &                    & 10000 100 20                                                  \\
            \bench{\shbfs}   &                    &                                                               \\
            \bench{\strmcls} &                    & 10 20 256 512 512 1000 none sc$\_$gpu$\_$output.out 1         \\
            \bench{\tfred}   &                    & --threads=128 --b=655360                                      \\
        \end{tabular}
        \caption{Benchmark setup. \hilite{Grid size for bar bench pending.}}
        \label{tab:stats}
    \end{table}
\end{small}


==> tab-compressed.tex <==
\begin{small}
    \begin{table*}
        \centering
        \begin{tabular}{lrrr|rr||r|rr|rr}
                             & \multicolumn{5}{c||}{\textbf{Execution time (s)}} & \multicolumn{5}{c}{\textbf{Memory Overhead (MB)}}                                                                                              \\
                             & \textbf{BC+}                                      & \textbf{\scord}                                   & \textbf{\appc} & \textbf{BC+-CMP} & \textbf{\appcc} & \bc & \scord & \bcc & \appc & \appcc \\
            \toprule
            \bench{\conv}    & 0.80                                              & 0.79                                              & 0.79           & 0.81             & 0.79                                                   \\
            \bench{\mm}      & 5.52                                              & 5.68                                              &                & 4.84             & 31.02                                                  \\
            \bench{\red}     & 0.50                                              & 0.51                                              & 0.51           & 0.50             & 0.51                                                   \\
            \bench{\ruleone} & 7.11                                              & 6.85                                              & 7.74           & 7.01             & 8.25                                                   \\
            \bench{\uts}     & 1.74                                              & 0.64                                              &                & 0.81                                                                      \\
        \end{tabular}
        \caption{Comparison of the memory overheads (in MiB) of the different dynamic analyses.}
        \label{tab:mem-overhead}
    \end{table*}
\end{small}


==> tab-data-races.tex <==
\begin{small}
    \begin{table}
        \centering
        \begin{tabular}{lrrrrr}
                              & \textbf{Total} & \textbf{BC+} & \textbf{SRD} & \textbf{GP} & \textbf{iGuard} \\
            \toprule
            \bench{\conv}     & 5               & 5            & 5            & 5           & 5               \\
            \bench{\red}      & 19               & 19           & 2            & 19          & 12              \\
            \bench{\ruleone}  & 30              & 30           & 24           & 30          & 5               \\
            % \bench{\mm}       & 2              & 2             & 1             & 2            \\
            \bench{stencil}   & 2              & 1            & 0            & 2           & 0               \\

            \midrule

            \bench{\hotspot}  & 0               & 0            & 0            & 0           & 0               \\
            \bench{\kmeans}   & 0               & 0            & 0            & 0           & 0               \\
            \bench{\needle}   & 0               & 0            & 0            & 0           & 0               \\
            \bench{thrfenred} & 34               & 31           & 6            & 34          & 0               \\
            \bench{\pf}       & 5               & 2            & 2            & 5           & 0               \\
            \bench{shocbfs}   & 4               & 4            & 3            & 4           & 2               \\

            %            \bench{strmcls}   &              &              &             \\
            %            \bench{\uts}     &                &               &              &             \\
        \end{tabular}
        \caption{Comparison of the number of unique kinds of data races detected by the different dynamic analyses on our benchmarks.}
        \label{tab:data-races}
    \end{table}
\end{small}


==> tab-merged.tex <==
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}

\begin{small}
    \begin{table*}
        \centering
        \begin{tabular}{lr|rr|r|rrr|rr||rrrrr}
                              & \multicolumn{9}{c}{\textbf{\normalsize Run-time Performance (s)}} & \multicolumn{5}{c}{\textbf{\normalsize Peak Memory Overhead (MB)}}                                                                                                                                                                                                \\
                              & \textbf{UM}                                                       & \textbf{NVB}                                                       & \textbf{BLK} & \textbf{iGuard} & \textbf{SRD} & \textbf{BC+} & \textbf{GP} & \textbf{BC+-CP} & \textbf{GP-CP} & \textbf{SRD} & \textbf{BC+} & \textbf{BC+-CP} & \textbf{GP} & \textbf{GP-CP} \\
            \toprule
            \bench{\conv}     & 0.83                                                              & 0.8                                                                & 1.18         & 7.73            & 6.53         & 10.6         & 14.7        & 11.63           & 47.69          & 494          & 1987         & 742             & 1049        & 1052           \\
            \bench{\mm}       & --                                                                & --                                                                 & --           & --              & --           & --           & --          & --              & --                                                                                            \\
            \bench{\red}      & 3.18                                                              & 3.18                                                               & 3.42         & 3.59            & 18.01        & 21.93        & 42.42       & 21.24           & 47.75          & 5016         & 6822         & 6626            & 10580       & 10218          \\
            \bench{\ruleone}  & 0.65                                                              & 0.65                                                               & 1.58         & 1.29            & 26.7         & 24.48        & 48.76       & 44.47           & 103.17         & 1065         & 2069         & 2092            & 3575        & 3570           \\
            \bench{\uts}      & --                                                                & --                                                                 & --           & --              & --           & --           & --          & --              & --                                                                                            \\
            \midrule
            \bench{\hotspot}  & 0.35                                                              & 0.35                                                               & 0.62         & 0.67            & 3.2          & 126.84       & 232.28      & 187.41          & 517.57         & 505          & 5575         & 861             & 2126        & 1338           \\
            \bench{\kmeans}   & 1.71                                                              & 1.75                                                               & 11.82        & 2.8             & 41.03        & 64.46        & 210.48      & 426.09          & 1709.39        & 6580         & 6445         & 6360            & 11013       & 1100           \\
            \bench{\needle}   & 0.21                                                              & 0.26                                                               & 67.95        & 1.16            & 79.05        & 110.77       & 152.48      & 159.65          & 310.98         & 1747         & 1823         & 1829            & 3057        & 3074           \\

            \bench{\pf}       & 0.23                                                              & 0.22                                                               & 1.55         & 0.54            & 3.18         & 32.63        & 95.41       & 25.27           & 52.04          & 305          & 495          & 397             & 758         & 546            \\
            \bench{strmcls}   & 0.28                                                              & 0.31                                                               & 373.74       & 12.17           & 393.74       & 398.93       & 420.52      & 412.91          & 425.85         & 138          & 476          & 477             & 469         & 496            \\
            \bench{thrfenred} & 0.22                                                              & 0.24                                                               & 25.99        & 0.99            & 39.41        & 51.37        & 88.74       & 61.73           & 122.07         & 238          & 327          & 287             & 419         & 378            \\
            \bench{shocbfs}   & 0.18                                                              & 0.21                                                               & 26.08        & 0.7             & 25.77        & 26.85        & 26.34       & 26.4            & 26.14          & 120          & 120          & 120             & 120         & 120            \\
            \bottomrule
            \textbf{geomean}  & 0.47                                                              & 0.49                                                               & 8.12         & 1.79            & 23.0         & 49.73        & 85.65       & 68.81           & 146.55                                                                                        \\
        \end{tabular}
        \swarnendu{SB will split the table into two.}
        \caption{Comparison of the run times (in seconds) of the different dynamic analyses.}
        \label{tab:perf-overhead}
    \end{table*}
\end{small}


==> tab-stats.tex <==
\begin{small}
    \begin{table*}
        \centering
        \begin{tabular}{lrrrrrrrr}
                             & \multicolumn{2}{c}{\textbf{Memory accesses}}
                             & \multicolumn{2}{c}{\textbf{Lock operations}}
                             & \multicolumn{2}{c}{\textbf{Atomic operations}}
                             & \multicolumn{2}{c}{\textbf{Fence operations}}                                                                   \\
            % \cline{2-3}
            % \cline{4-5}
            % \cline{6-7}
                             & Reads & Writes  & Acquires & Releases & Block   & Device & Block & Device \\
            \toprule
            \bench{\conv}    & 17999960 & 1000000 & 0        & 0        & 8999980 & 0      & 0     & 0      \\
            \bench{\mm}      &                                                &        &          &          &       &        &       &        \\
            \bench{\red}     & 25631262 & 40703   & 0        & 0        & 24224 & 30   & 883     & 0       \\
            \bench{\ruleone} & 62499990 & 37500000       & 0         & 0         & 232070  & 306      &  8374     & 156       \\
            \bench{\uts}     &          &        &          &          &       &        &       &        \\
            \bench{stencil}  & 930      & 136       & 256         & 32         & 0      & 480       & 0      & 224       \\

            \midrule

            \bench{\hotspot} &  5246320        & 2159520       &  0        & 0         &  0     & 0       &  0     &  0      \\
            \bench{\kmeans}  &  16796680        &  35075420      &  0        &  0        & 0      &  0      & 0      &  0      \\
            \bench{\needle}  & 25706496         & 13123584       &  0        &   0       &   0    &   0     &   0    &   0     \\
            \bench{\pf}      & 5435620  & 2209690       & 0         &   0       & 0      &  0      & 0      &  0      \\
            \bench{\shbfs}   & 3879960         & 19980       & 0         &  0        &  0     &  0      &  0     &  0      \\
            \bench{\strmcls} & 378935408         & 853904       & 0         &  0        &  0     &  0      &  0     &  0      \\
            \bench{\tfred}   & 68703908         &  2533640      & 0         & 0         & 0      & 6400       &  0     & 25600       \\
        \end{tabular}
        \caption{Run-time statistics for the benchmarks.}
        \label{tab:stats}
    \end{table*}
\end{small}


==> usm.tex <==
\section{Unified Shared Memory}
\label{sec:usm}

Typically, execution of  GPU kernels happen using the following four steps:
\begin{itemize}
    \item Allocate  memory on the device,
    \item Copy relevant data from the host to device,
    \item Launch the kernel; the results are generated on the device (GPU) memory,
    \item Copy results back to host.
\end{itemize}

Recent GPU architectures have introduced the concept of Unified Shared Memory (USM)~\cite{cuda-pg}. USM refers to a single memory space accessible from both the host and the device. The CUDA runtime and hardware takes care of migrating data when required. This leads to the potential for a new form of races that have not been covered before, a race between a host thread and a device thread. The ScoRD algorithm, primarily dealing with fences and locksets inside the kernel, will clearly not suffice to detect such cross device races. However, we believe Barracuda's technique of shifting the race detection to the host through buffers can be used to detect these kinds of races. Of course, newer system level synchronization operations will now have to be considered as well.

We have two ways of analysing races on USM code, which are discussed below.

\subsection{Collision-based solutions}

This technique has the benefit of being applicable universally, regardless of synchronization primitives. However, while in CPU domain, memory watchpoints can be used to monitor accesses to a specific memory location, such a provision is not available in current GPUs and thus every memory access needs to be monitored to verify the access against a list of memory addresses that we are currently interested in. This can lead to very large performance overheads. Also, by their very nature, collision based techniques have the possibility of false negatives if an appropriately large delay is not chosen.

\subsection{Vector clock solutions}

This approach would require us to collect traces from both device and host threads simultaenously. While this is a more elegant solution, vector clock based solutions will require encoding the semantics of complicated synchronization operations and even with that, will fail to hold up if newer synchronization primitives are added or if the existing ones have a change in functionality.

% \swarnendu{Add a few lines about the pros and cons with vector clocks and collision analysis. Also discuss whether existing Barracuda and ScoRD techniques will work for USM or not.}
% \sagnik{Sections addressing these points have been added.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

